Machine learning attack on copy detection patterns: are 1x1 patterns cloneable?

Nowadays, the modern economy critically requires reliable yet cheap protection solutions against product counterfeiting for the mass market. Copy detection patterns (CDP) are considered as such solution in several applications. It is assumed that being printed at the maximum achievable limit of a printing resolution of an industrial printer with the smallest symbol size 1x1 elements, the CDP cannot be copied with sufficient accuracy and thus are unclonable. In this paper, we challenge this hypothesis and consider a copy attack against the CDP based on machine learning. The experimental based on samples produced on two industrial printers demonstrate that simple detection metrics used in the CDP authentication cannot reliably distinguish the original CDP from their fakes. Thus, the paper calls for a need of careful reconsideration of CDP cloneability and search for new authentication techniques and CDP optimization because of the current attack.

==> tab/dataset_tab.tex <==
% -------------------------
\begin{table*}[!hbt]
    
	\centering
	\renewcommand*{\arraystretch}{2}
	%
	\caption{The brief overview of the new datasets CDP which are created and investigated in this paper. \textit{Digital} codes are both \textit{original} and \textit{estimated} templates, original codes are printed \textit{original} templates and \textit{fake} codes are printed \textit{estimated} templates.}
	\label{tab:dataset}
	{\small
	\begin{tabular}{m{0.03\linewidth}m{0.08\linewidth}m{0.22\linewidth}m{0.15\linewidth}m{0.15\linewidth}m{0.19\linewidth}} \hline
	\# & Name & Digital templates & Printing & Acquisition & \# of codes \\ \hline
    %
    % CSGC
    %
	 \multicolumn{1}{m{0.03\linewidth}}{
	 (1)
	 } & 
	 \multicolumn{1}{m{0.08\linewidth}}{
	 CDP55
	 } & 
	 \multicolumn{1}{m{0.22\linewidth}}{ 
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
                \item[] size: $228 \times 228$
                \item[] symbol size: $1 \times 1$
                \item[] densities: $30,35,40,45,50$
            \end{itemize}  
            }    
		& \multicolumn{1}{m{0.15\linewidth}}{
			\textit{Offset}, at 812.8 dpi: 
        	\begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=0pt]
        		\item[] $\boldsymbol{\cdot}$ HP Indigo 5500
    	    \end{itemize}
            }    
		& \multicolumn{1}{>{\centering\arraybackslash}m{0.15\linewidth}}{ 
            \begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=1pt]
            	\item[] \textit{Scanner}:            
                \item[] $\boldsymbol{\cdot}$ Epson V850 Pro
                \item[] $\;\;$ at 2400 ppi
                \item[] $\;\;$ at 6400 ppi                                
            \end{itemize}  
            }
		& \multicolumn{1}{m{0.19\linewidth}}{
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=3pt]
                \item[] digital original: 3600
                \item[] digital fakes: 1440
                \item[] scanned original: 4320
                \item[] scanned fakes: 1440
                \item[] total: 6480
            \end{itemize}  
            }                    
     \\[-0.35cm] \hline
     
    \multicolumn{1}{m{0.03\linewidth}}{
	 (2)
	 } & 
	 \multicolumn{1}{m{0.08\linewidth}}{
	 CDP76
	 } & 
	 \multicolumn{1}{m{0.22\linewidth}}{ 
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=0pt]
                \item[] size: $228 \times 228$
                \item[] symbol size: $1 \times 1$
                \item[] densities: $30,35,40,45,50$
            \end{itemize}  
            }    
		& \multicolumn{1}{m{0.15\linewidth}}{
			\textit{Offset}, at 812.8 dpi: 
        	\begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=0pt]
        		\item[] $\boldsymbol{\cdot}$ HP Indigo 7600
    	    \end{itemize}
            }    
		& \multicolumn{1}{>{\centering\arraybackslash}m{0.15\linewidth}}{ 
            \begin{itemize}[leftmargin=0.2cm,noitemsep,topsep=1pt]
            	\item[] \textit{Scanner}:            
                \item[] $\boldsymbol{\cdot}$ Epson V850 Pro
                \item[] $\;\;$ at 2400 ppi
                \item[] $\;\;$ at 6400 ppi                                
            \end{itemize}  
            }
		& \multicolumn{1}{m{0.19\linewidth}}{
            \begin{itemize}[leftmargin=0cm,noitemsep,topsep=3pt]
                \item[] digital original: 3600
                \item[] digital fakes: 1440
                \item[] scanned original: 4320
                \item[] scanned fakes: 1440
                \item[] total: 6480
            \end{itemize}  
            }                    
     \\[-0.35cm] \hline    
	\end{tabular}
	}
\end{table*}
% -------------------------

==> tab/svm1_all_tab.tex <==
\begin{table}

\centering
\renewcommand*{\arraystretch}{1.2}

\caption{The results of the one-class SVM training using all metrics. $P_D$ indicates the printer used for the originals and $P_A$ is the attacker's printer. Both $P_{miss}$ and $P_{fa}$ are calculated over test subset.}
\label{tab:svm1all}
\begin{tabular}[t]{cccc}
\toprule
$P_D$ & $P_A$ & $P_{miss}$ & $P_{fa}$ \\
\midrule
HPI55 & HPI55 & $\mathbf{15.67 \:(\pm3.29)}$ & $\mathbf{6.54\:(\pm3.47)}$ \\
HPI55 & HPI76 & $100.0 \:(\pm0.0)$ & $0.0\:(\pm0.0)$ \\
\cline{1-4}
HPI76 & HPI55 & $100.0 \:(\pm0.0)$ & $22.21\:(\pm5.82)$ \\
HPI76 & HPI76 & $\mathbf{12.0 \:(\pm2.74)}$ & $\mathbf{0.0\:(\pm0.0)}$ \\
\bottomrule

\end{tabular}
\vspace{-5mm}
\end{table}

==> tab/svm1_pairs_tab.tex <==
\begin{table}[t!]
\renewcommand*{\arraystretch}{1.2}
\centering

\caption{The results of the one-class SVM training using pairs of metrics $M_1,\:M_2$. $P_D$ indicates the original CDP printer subset and $P_A$ the fake CDP printer.}
\label{tab:svm1pairs}
\begin{tabular}{ccccc}
\toprule
$M_1, M_2$ & $P_D$ & $P_A$ & $P_{miss}$ & $P_{fa}$ \\
\midrule
\multirow{4}{*}{\shortstack[c]{CORR \\ JACCARD}} 
& HPI55 &  HPI55 & $\mathbf{14.03\:(\pm5.16)}$ & $\mathbf{18.92\:(\pm7.06)}$ \\   & HPI55 &  HPI76 & $64.19\:(\pm4.47)$ & $5.31\:(\pm6.26)$ \\
\cline{2-5}
& HPI76 &  HPI55 & $98.06\:(\pm1.4)$ & $27.42\:(\pm8.25)$ \\  
& HPI76 &  HPI76 & $\mathbf{11.06\:(\pm2.13)}$ & $\mathbf{18.79\:(\pm8.98)}$ \\
% \cline{1-4}
% \multirow{2}{*}{HAMMING, CORR} & HPI55 &  $\mathbf{13.36\:(\pm3.66)\:/\:17.5\:(\pm8.32)}$ &     $94.19\:(\pm7.74)\:/\:0.0\:(\pm0.0)$ \\
%               & HPI76 &  $99.58\:(\pm0.22)\:/\:26.33\:(\pm5.33)$ &     $\mathbf{10.22\:(\pm0.84)\:/\:0.0\:(\pm0.0})$ \\
% \cline{1-4}
% \multirow{2}{*}{HAMMING, JACCARD} & HPI55 &  $\mathbf{13.31\:(\pm3.15)\:/\:12.08\:(\pm4.71)}$ &     $99.17\:(\pm1.71)\:/\:0.0\:(\pm0.0)$ \\
%               & HPI76 &     $100.0\:(\pm0.0)\:/\:20.9\:(\pm3.3)$ &     $\mathbf{10.89\:(\pm2.23)\:/\:0.0\:(\pm0.0)}$ \\
\cline{2-5}
\hline
\multirow{4}{*}{\shortstack[c]{HAMMING \\ SSIM}} 
& HPI55 &  HPI55 &  $\mathbf{12.58\:(\pm1.55)}$ & $\mathbf{2.62\:(\pm2.34)}$ \\
& HPI55 &  HPI76 &  $99.53\:(\pm0.62)$ & $0.0\:(\pm0.0)$ \\
\cline{2-5}
& HPI76 & HPI55 &   $100.0\:(\pm0.0)$ & $35.11\:(\pm7.65)$ \\     
& HPI76 & HPI76 & $\mathbf{9.97\:(\pm0.78)}$ & $\mathbf{0.4\:(\pm0.44)}$ \\
% \cline{1-4}
% \multirow{2}{*}{SSIM, CORR} & HPI55 &  $14.03\:(\pm3.32)\:/\:83.51\:(\pm3.49)$ &   $38.75\:(\pm6.7)\:/\:34.78\:(\pm6.14)$ \\
%               & HPI76 &  $40.89\:(\pm5.03)\:/\:42.14\:(\pm7.45)$ &   $11.92\:(\pm1.02)\:/\:10.28\:(\pm5.5)$ \\
% \cline{1-4}
% \multirow{2}{*}{SSIM, JACCARD} & HPI55 &  $14.42\:(\pm3.88)\:/\:78.35\:(\pm4.14)$ &     $51.5\:(\pm4.6)\:/\:0.58\:(\pm0.87)$ \\
%               & HPI7\label{tab:svm1pairs}6 &  $82.42\:(\pm1.38)\:/\:28.83\:(\pm5.38)$ &   $12.11\:(\pm1.07)\:/\:1.04\:(\pm0.97)$ \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

==> tab/svm2_all_tab.tex <==
\begin{table}
\centering
\renewcommand*{\arraystretch}{1.2}
\caption{The results of the supervised two-class SVM training using all metrics. $P_D$ indicates the printer of the training subset and $P_A$ the printer of the test subset.}
\label{tab:svm2all}
\begin{tabular}[t]{ccccc}

\toprule
Trained on & $P_D$ & $P_A$ & $P_{miss}$ & $P_{fa}$ \\
\midrule
\multirow{2}{*}{$\x^{55}$, $\f^{55/55}$}
& HPI55 & HPI55 &  $\mathbf{3.19\:(\pm1.09)}$ & $\mathbf{1.42\:(\pm1.16)}$ \\
& HPI55 & HPI76 & $61.58\:(\pm5.41)$ & $0.5\:(\pm0.61)$ \\
\cline{1-5}
\multirow{2}{*}{$\x^{55}$, $\f^{55/76}$}
& HPI55 & HPI55 & $2.28\:(\pm0.59)$ & $3.39\:(\pm2.79)$ \\
& HPI55 & HPI76 & $48.53\:(\pm1.42)$ & $3.67\:(\pm2.1)$ \\
\cline{1-5}
\multirow{2}{*}{$\x^{76}$, $\f^{76/55}$}
& HPI76 & HPI55 & $3.06\:(\pm6.6)$ & $95.65\:(\pm5.69)$ \\
& HPI76 & HPI76 & $0.14\:(\pm0.2)$ & $0.31\:(\pm0.22)$ \\
\cline{1-5}
\multirow{2}{*}{$\x^{76}$, $\f^{76/76}$}
& HPI76 & HPI55 & $0.0\:(\pm0.0)$ & $99.26\:(\pm1.61)$ \\
& HPI76 & HPI76 & $\mathbf{0.06\:(\pm0.12)}$ & $\mathbf{0.17\:(\pm0.2)}$ \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\end{table}
